Transparent Spheres as Gravitational Lens

In this contribution, we present a short account of gravitational lenses and how to calculate different properties of its images in the case of having a transparent distribution of matter such as the uniform transparent sphere, isothermal gas sphere, non-singular isothermal gas sphere and a transparent King profile. With the help of XFGLenses software, and numerical methods, different images arising from all of these profiles, and the different caustics and critical curves are shown. The images were consistent with several previous results that are expected for transparent profiles, like having an odd number of images, and reducing the number of images by two when the source passes through the caustic. The curves shown in the caustics where the diamond, the ellipse and the lemniscate-like. For the critical curves, the most common curve was the ellipse, and the lemniscate appeared in the transparent NSIS case, which is consistent with the fact that these curves are common in gravitational lenses.

==> Time_delay_and_magnification.tex <==

\subsection{Magnification}

The light that passes through a gravitational lens undergoes a change of direction that causes phenomena such as distortion of the image in size and shape. This is mainly due to the mass distribution of the lens.
\\
\\
The magnification of a small source is given by:
\begin{equation}
    \mathbf{M} = \frac{1}{det(\mathbf{J})}
\end{equation}





\subsection{Time delay}

The delay time represents the difference in the paths of light rays emitted by a source that generates multiple images through a lens system. 
To consider a time delay, two different components must be taken into account.
\\
\\
One of them is that a ray of light that travels a curved path takes more time to propagate than a ray that travels in a straight path (without the presence of a gravitational field), this is what is known as the Shapiro effect.
\\
\\
The second thing to consider is that the individual light rays that are emitted with different angles, which causes each of them to suffer a different curvature when passing through a lens system, this will cause each one to suffer different travel times.
\\
\\
Therefore, the total time delay will be the sum of both effects. One way to approximate the time delay for mass distributions of the form $r^{-n}$ is by means of the power series:

\begin{equation}
    \Delta t(n) = (n-1)\Delta t_{SIS}\Bigg[1-\frac{(2-n)}{12}\Bigg(\frac{\delta \theta}{ \langle \theta \rangle}\Bigg)^{2}+\cdots\Bigg]
\end{equation}

$\Delta t_{SIS}$, $\langle \theta \rangle$, $\delta \theta$  are given by

\begin{equation}
    \Delta t_{SIS}= \tau_{B}-\tau_{A} = \frac{1}{2}\frac{D_{d}D_{s}     }{cD_{ds}     }(\theta_{A}^{2}-\theta_{B}^{2})
\end{equation}

\begin{equation}
   \langle \theta \rangle = \frac{\theta_{A}+\theta_{B}   }{2}
\end{equation}

\begin{equation}
   \delta \theta = \frac{\theta_{A}-\theta_{B}   }{2}
\end{equation}

==> codigo.tex <==
\usepackage[usenames,dvipsnames]{pstricks}
\usepackage{pstricks-add}
\usepackage{epsfig}
\usepackage{pst-grad} % For gradients
\usepackage{pst-plot} % For axes
\usepackage[space]{grffile} % For spaces in paths
\usepackage{etoolbox} % For spaces in paths
\makeatletter % For spaces in paths
\patchcmd\Gread@eps{\@inputcheck#1 }{\@inputcheck"#1"\relax}{}{}
\makeatother
 
 

 
 \begin{document}
 

 
 
\begin{figure}
\psscalebox{1.0 1.0} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-6.6828413)(10.955,5.092841)
\psline[linecolor=black, linewidth=0.03](3.9085498,2.6610603)(0.78007454,1.5944357)(8.00609,1.4887662)(10.261326,2.6211374)(3.9085498,2.674368)(3.9085498,2.674368)
\psline[linecolor=black, linewidth=0.03, linestyle=dotted, dotsep=0.10583334cm](0.73588514,3.0878515)(0.6574988,-6.5844083)(0.47655898,-6.6578417)
\psline[linecolor=black, linewidth=0.03, linestyle=dotted, dotsep=0.10583334cm](3.9083605,4.390132)(3.9308488,-5.319962)(3.9533372,-5.357671)
\psline[linecolor=black, linewidth=0.03, linestyle=dotted, dotsep=0.10583334cm](7.8888025,4.2958593)(8.316081,-6.243835)
\psline[linecolor=black, linewidth=0.03, linestyle=dotted, dotsep=0.10583334cm](10.205105,4.427841)(10.4075,-6.0552893)(10.4075,-6.0552893)
\psline[linecolor=black, linewidth=0.03](3.8608305,0.30419606)(0.8246171,-0.90144014)(8.1186905,-1.2156298)(10.287851,0.051158853)(3.8386683,0.30419606)(3.858463,0.27390498)
\psline[linecolor=black, linewidth=0.03](3.838493,-1.9798409)(0.7375,-3.3742824)(8.223725,-3.6741717)(10.360121,-2.2473667)(3.838493,-1.9798409)
\psline[linecolor=black, linewidth=0.02, linestyle=dashed, dash=0.17638889cm 0.10583334cm](5.6409492,-2.456076)(5.715621,2.1704528)(5.715621,2.1704528)
\psline[linecolor=black, linewidth=0.02](5.715621,-0.55629355)(7.9557753,-0.24338824)(7.9557753,-0.2657386)
\psline[linecolor=black, linewidth=0.02](5.715621,2.1704528)(6.9850416,2.2598543)
\psline[linecolor=black, linewidth=0.02, linestyle=dashed, dash=0.17638889cm 0.10583334cm](5.6409492,-2.456076)(5.6160583,-3.0371857)
\psline[linecolor=black, linewidth=0.02, linestyle=dashed, dash=0.17638889cm 0.10583334cm](5.6160583,-2.9477842)(6.960151,2.237504)(6.960151,2.237504)
\psline[linecolor=black, linewidth=0.02](5.6160583,-2.9701345)(7.9557753,-0.24338824)
\psline[linecolor=black, linewidth=0.02](7.930885,-0.24338824)(6.960151,2.2822046)
\psline[linecolor=black, linewidth=0.02, linestyle=dashed, dash=0.17638889cm 0.10583334cm](7.9557753,-0.22103786)(8.9514,0.9411819)(8.9514,0.9411819)
\psline[linecolor=black, linewidth=0.03](9.474102,2.1481025)(10.17104,2.125752)(10.146149,2.125752)
\psline[linecolor=black, linewidth=0.03](9.474102,-2.9254339)(10.071477,-2.9477842)(10.071477,-2.9477842)
\psline[linecolor=black, linewidth=0.03, linestyle=dashed, dash=0.17638889cm 0.10583334cm](9.822571,2.1034017)(9.747899,-2.880733)(9.747899,-2.880733)
\psline[linecolor=black, linewidth=0.03](8.702494,-3.5288942)(9.39943,-3.5512445)(9.39943,-3.5512445)
\psline[linecolor=black, linewidth=0.03](8.727385,-1.0033011)(9.349649,-1.0033011)(9.349649,-1.0033011)
\psline[linecolor=black, linewidth=0.03, linestyle=dashed, dash=0.17638889cm 0.10583334cm](9.100743,-1.0703523)(9.100743,-3.5959454)(9.100743,-3.5959454)
\psline[linecolor=black, linewidth=0.03](1.8077306,2.0123587)(1.0611433,2.037992)
\psline[linecolor=black, linewidth=0.03](1.8326867,-0.48924243)(1.0859685,-0.46689203)
\psline[linecolor=black, linewidth=0.03, linestyle=dashed, dash=0.17638889cm 0.10583334cm](1.4095464,1.9581242)(1.4593276,-0.3886657)
\rput[bl](4.2175,-0.5921588){Lens plane}
\rput[bl](4.0775,1.8478411){Source plane}
\rput[bl](4.4375,-2.972159){Observer}
\rput[bl](6.0375,2.267841){η}
\rput[bl](6.7375,-0.31215882){ξ}
\pscustom[linecolor=black, linewidth=0.03, linestyle=dashed, dash=0.17638889cm 0.10583334cm]
{
\newpath
\moveto(5.6575,-1.2721589)
\lineto(5.7675,-1.2921588)
\curveto(5.8225,-1.3021588)(5.8925,-1.3221588)(5.9075,-1.3321588)
\curveto(5.9225,-1.3421588)(5.9475,-1.3621588)(5.9575,-1.3721588)
}
\pscustom[linecolor=black, linewidth=0.03, linestyle=dashed, dash=0.17638889cm 0.10583334cm]
{
\newpath
\moveto(5.9575,-1.3521588)
\lineto(5.9775,-1.3721588)
\curveto(5.9875,-1.3821588)(6.0025,-1.4021589)(6.0175,-1.4321588)
}
\pscustom[linecolor=black, linewidth=0.03, linestyle=dashed, dash=0.17638889cm 0.10583334cm]
{
\newpath
\moveto(5.6575,-1.7921588)
\lineto(5.8375,-1.8121588)
\curveto(5.9275,-1.8221588)(6.0475,-1.8421588)(6.0775,-1.8521588)
\curveto(6.1075,-1.8621588)(6.1475,-1.8821588)(6.1575,-1.8921589)
\curveto(6.1675,-1.9021589)(6.1925,-1.9221588)(6.2075,-1.9321588)
\curveto(6.2225,-1.9421588)(6.2525,-1.9621588)(6.2675,-1.9721588)
\curveto(6.2825,-1.9821588)(6.3075,-2.0021589)(6.3175,-2.0121589)
\curveto(6.3275,-2.0221589)(6.3425,-2.0371587)(6.3575,-2.0521588)
}
\pscustom[linecolor=black, linewidth=0.03, linestyle=dashed, dash=0.17638889cm 0.10583334cm]
{
\newpath
\moveto(7.5975,0.70784116)
\lineto(7.6475,0.7278412)
\curveto(7.6725,0.7378412)(7.8075,0.7478412)(7.9175,0.7478412)
\curveto(8.0275,0.7478412)(8.1675,0.7378412)(8.1975,0.7278412)
\curveto(8.2275,0.7178412)(8.2875,0.69784117)(8.3175,0.6878412)
\curveto(8.3475,0.6778412)(8.4025,0.6578412)(8.4275,0.6478412)

\end{figure}


 \end{document}

==> codigo1.tex <==

\begin{figure}
\psscalebox{1.0 1.0} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-4.08)(9.230761,-0.64)
\definecolor{colour0}{rgb}{0.6,0.6,0.6}
\psdots[linecolor=black, dotsize=0.022](1.72,-2.34)
\pscircle[linecolor=black, linewidth=0.04, fillstyle=solid, dimen=outer](1.72,-2.34){1.72}
\pscircle[linecolor=black, linewidth=0.04, fillstyle=solid,fillcolor=colour0, dimen=outer](1.72,-2.34){0.82}
\psline[linecolor=black, linewidth=0.04, fillstyle=solid,fillcolor=colour0]{<->}(1.72,-2.34)(2.46,-2.1)(2.46,-2.1)
\psline[linecolor=black, linewidth=0.04, fillstyle=solid,fillcolor=colour0]{<->}(1.72,-2.34)(2.2,-3.96)(2.24,-3.94)
\pscircle[linecolor=black, linewidth=0.04, fillstyle=solid, dimen=outer](6.64,-2.34){1.72}
\psline[linecolor=black, linewidth=0.04, linestyle=dashed, dash=0.17638889cm 0.10583334cm, fillstyle=solid](4.6163635,-2.34)(9.196363,-2.3945456)(9.196363,-2.3945456)(9.196363,-2.4145455)
\psline[linecolor=black, linewidth=0.04, fillstyle=solid](5.14,-1.68)(8.12,-1.72)(8.12,-1.72)
\psline[linecolor=black, linewidth=0.04, fillstyle=solid](5.16,-2.96)(8.14,-2.96)(8.14,-2.94)
\psline[linecolor=black, linewidth=0.04, fillstyle=solid]{<->}(4.702424,-2.2175)(4.702424,-1.84)
\psline[linecolor=black, linewidth=0.04, linestyle=dashed, dash=0.17638889cm 0.10583334cm, fillstyle=solid](6.5995784,-0.73774004)(9.220422,-0.78225994)(9.220422,-0.78225994)
\psline[linecolor=black, linewidth=0.04, fillstyle=solid]]{<->}(9.1620455,-0.9175)(9.1620455,-2.2675)(9.1620455,-2.2675)
\end{pspicture}
}
\end{figure}
